Domain-Adaptive Device Fingerprints for Network Access Authentication Through Multifractal Dimension Representation

RF data-driven device fingerprinting through the use of deep learning has recently surfaced as a potential solution for automated network access authentication. Traditional approaches are commonly susceptible to the domain adaptation problem where a model trained on data from one domain performs badly when tested on data from a different domain. Some examples of a domain change include varying the device location or environment and varying the time or day of data collection. In this work, we propose using multifractal analysis and the variance fractal dimension trajectory (VFDT) as a data representation input to the deep neural network to extract device fingerprints that are domain generalizable. We analyze the effectiveness of the proposed VFDT representation in detecting device-specific signatures from hardware-impaired IQ signals, and evaluate its robustness in real-world settings, using an experimental testbed of 30 WiFi-enabled Pycom devices under different locations and at different scales. Our results show that the VFDT representation improves the scalability, robustness and generalizability of the deep learning models significantly compared to when using raw IQ data.

==> Comments.tex <==
%%% 6/8/22
- add a couple of sentences at the begining of each section (e.g., Sec V.) introducuing the scope of the section

section: experimental setup
- [DONE] DNN section needs to be moved to Results section
- [DONE] exprimental scenarios: put in a table could be better; there is some redundacy with Same Tx, Different Tx etc.

section: results:
- [DONE] did you define what 'vanilla' model is?
- [DONE] caption of subfigure should be done via caption, not adding (a) etc. Did fig 13

NOTES:

I have modified the `closed-set' evaluation sections (hardware, channel, and configuration portability). >>>Let me know if these parts need further work.<<<

I have removed the background section in favor of integrating the background into the 'proposed technique' section. 

I also removed the background information on the hardware impairments...this is because they have been well covered in other works on RF fingerprinting, and my work does not rely on the particular extraction of one kind of impairment (was excessive background for my technique)


I still need to:
- Edit the `open-set' evaluation section (I plan on making this similar to the current `closed-set' section)
- Edit the first few paragraphs of the 'proposedtechnique.tex' section (needs to reflect changes in this section)


==> related.tex <==


%main structure for section

%some look at preprocessing

%some look calibrating model itself

%some look at only scalability and real world 

%some look at deep fingerprint analysis but then no domain (other fractal dimension paper)

%

Existing works attempting to overcome the domain adaptation problem focus on a variety of methods. Some look at using a certain type of preprocessing to extract a single, specific hardware feature, such as the CFO, for example \cite{joo2020hold}. Others use various custom types of preprocessing to help extract an overall fingerprint, independent of domain, that is then passed through a deep learning model for classification \cite{9732439}, \cite{shen2021scalable}. There are also attempts to directly calibrate the model itself to overcome portability problems across domains \cite{gaskin2022tweak}. 

Aside from focusing on domain adaptation, related works also approach other issues with device fingerprinting including scalability \cite{9771750} and signal interference \cite{10.1145/3522783.3529520}. Alternatively, \cite{10012578} proposes using a more complex device fingerprint by combining several different features, including the fractal dimension which is a component of multifractal analysis, for use in a deep learning model. While they consider basic channel noise, complex domain adaptation is not explored. This work looks at analysis of the fundamental device fingerprint with multifractal analysis while also exploring its robustness across domains and scale. 
